Top quark pair production cross-section results at LHC in final states with tau or no leptons

ATLAS and CMS measured the top quark pair production inclusive cross section using proton-proton collision data collected at 7 TeV c.m. energy at the LHC during the year 2011 in several channels. This article presents the measurements of the cross section using selections of top quark pair production events with one hadronically decaying {\tau} lepton or no leptons at all.

==> Makefile <==
LATEX    = latex
DVIPS    = dvips

BASENAME = atlas-phys-proc-2013-081 

default: testlatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


